Structure is information: structural identifiability mappings for machine learning with partially observed dynamical systems

The successful application of modern machine learning for time series classification is often hampered by limitations in quality and quantity of available training data. To overcome these limitations, domain knowledge can be leveraged in the form of parameterised mechanistic dynamical models, whereby time series observations may be represented as instances of a predefined class of dynamical systems. Provided the dynamical models are interpretable in terms of domain-specific variables and their dynamic interaction, the learning process becomes interpretable as well and enables the modeller to handle sparsely and irregularly sampled data naturally. However, the internal processes of a dynamical model are often only partially observed. This can lead to ambiguity regarding which particular model realization best explains a given time series observation. This problem is well-known in the literature, and a dynamical model with this issue is referred to as structurally unidentifiable. Training a classifier that ignores knowledge about a structurally unidentifiable dynamical model can negatively influence classification performance. To address this issue, we employ structural identifiability analysis to explicitly relate parameter configurations that are associated with identical system outputs. Using the derived relations in classifier training, we demonstrate that this method significantly improves the classifier's ability to generalize to unseen data on a number of example models from the biomedical domain. This effect is especially pronounced when the number of training instances is limited. Our results demonstrate the importance of structural identifiability, a topic that has received relatively little attention from the machine learning community.

==> Acknowledgements.tex <==
\section*{Acknowledgment}
\begin{wrapfigure}[8]{L}{0.2\columnwidth}
\vspace{-0.35cm}
% \fbox{
\includegraphics[width=\linewidth]{final_version/manuscript/Figures/NWO logo - full colour - CMYK - clear space included.pdf}
% }
\end{wrapfigure}
\noindent This publication is part of the project \emph{Mechanistic machine learning: combining the explanatory power of dynamic models with the predictive power of machine learning} with file number VI.Vidi.193.098 of the research programme Vidi ENW, %[name research programme] 
which is %(partly) 
financed by the Dutch Research Council (NWO) under the grant \emph{NWO Talent Programme Vidi NWO Science domain 2019}. P.
Ti\v{n}o was supported by the EPSRC Prosperity Partnerships
grant ARCANE, EP/X025454/1.
%[grant id https ://doi.org/10.61686/#####].
% -> https://www.nwo.nl/en/grant-id
\noindent The authors would like to thank Sayali Bhatkar for providing parts of the structural identifiability analysis leading to the simplified expressions for the CML model.

% Template
%This publication is part of the project [name project] with file number [insert file number] of the research programme  which is (partly) financed by the Dutch Research Council (NWO) under the grant [grant id https ://doi.org/10.61686/#####].

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.5\linewidth]{Figures/NWO_logo.jpg}
%     %\caption{Caption}
%     %\label{fig:enter-label}
% \end{figure}

==> Biography.tex <==
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)

% or if you just want to reserve a space for a photo:
% [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/Biography/JNorden.jpg}}]

\def\myWidth{1in}\def\myHeight{1.25in}

\begin{IEEEbiography}[{\includegraphics[width=\myWidth,height=\myHeight,clip,keepaspectratio]{JanisNorden.jpg}}]{Janis Norden} received the bachelor's and master's degrees in Mathematics from the University of Groningen, The Netherlands. There, he is currently working toward the PhD degree in the Intelligent Systems research group at the Faculty of Science and Engineering. His research interests include machine learning and dynamical systems theory.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=\myWidth,height=\myHeight,clip,keepaspectratio]{ElisaOostwal.jpg}}]{Elisa Oostwal} obtained a bachelor's degree in Physics and both a bachelor's and master's degree in Computing Science at the University of Groningen. During her studies, she conducted research on the statistical physics of learning. She continued at the University of Groningen as a PhD candidate in the Intelligent Systems research group, where she focused on combining machine learning with interpretable models such as dynamical systems. She is currently employed as a data scientist at Sogeti, working on projects for Gasunie involving, among others, time series clustering and the development of RAG systems.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=\myWidth,height=\myHeight,clip,keepaspectratio]{MichaelChappell.jpg}}]{Mike Chappell}
Mike Chappell (BSc, MSc, PhD in Mathematics, University of Warwick) is a Professor within the School of Engineering at the University of Warwick where he heads the Systems and Information Engineering Discipline Stream. 
He co-leads the Biomedical Engineering Institute within the School of Engineering and co-leads the Technology in Health theme within the University of Warwick’s Health Research Spotlight. 
He also heads the University’s Gait Laboratory. 
He has research expertise in the systems modelling and data analysis of biomedical, pharmacokinetic/pharmacodynamic, biological and Quantitative and Systems Pharmacology (QSP) processes. 
Much of his work relates to the application to these fields of techniques in system dynamics, non-linear systems, data analytics, control and system identification with particular expertise in structural and practical identifiability analyses. 
He has had close research collaboration with industry and hospital-based research groups for over 30 years, in particular, major pharma. 
He led the Marie Curie funded European Industrial Doctorate training network on Innovative Modelling for Pharmaceutical Advances through Collaborative Training (IMPACT) in collaboration with AstraZeneca and is a member of the Management Committee for the EPSRC/MRC funded QSP-UK network. 
He is also a member of the International Federation for Automatic Control (IFAC) Technical Committee 8.2 on Biological and Medical Systems.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=\myWidth,height=\myHeight,clip,keepaspectratio]{PeterTino.png}}]{Peter Ti\v{n}o}
(M.Sc. Slovak University of Technology, Ph.D. Slovak Academy of Sciences) 
%was a Fulbright Fellow with the NEC Research Institute, Princeton, NJ, USA, and a Post-Doctoral Fellow with the Austrian Research Institute for AI, Vienna, Austria, and with Aston University, Birmingham, UK. Since 2003, he 
%has been 
is with the School of Computer Science, University of Birmingham, %Edgbaston, Birmingham, UK, 
%since 2003 
where he is currently a Full Professor-Chair in Complex and Adaptive Systems. His current research interests include dynamical systems, machine learning, probabilistic modelling of structured data, evolutionary computation, and fractal analysis. Peter was a recipient of the U.K.- Hong-Kong Fellowship for Excellence in 2008, three Outstanding Paper of the Year Awards from the IEEE Trans. on Neural Networks in 1998 and 2011 and the IEEE Trans. on Evolutionary Computation in 2010, and the Best Paper Award at ICANN 2002. 
%He serves on the editorial boards of several journals.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=\myWidth,height=\myHeight,clip,keepaspectratio]{kerstin-bunte-2025.jpg}}]{Kerstin Bunte} %graduated at the Faculty of Technology at the University of Bielefeld, Germany, She 
is a professor of machine learning for interdisciplinary data science at the Bernoulli Institute for Mathematics, Computer Science and Artificial Intelligence at the University of Groningen, The Netherlands. % since July 2016. 
%She received her Ph.D. in Computer Science in 2011 from the University of Groningen. 
%She had research visits at the University of Rochester (USA) and postdoctoral positions have taken her to Bielefeld University (Germany), Aalto University (Finland), and Université catholique de Louvain (Belgium). 
She received her Ph.D. in Computer Science in 2011 in Groningen, had 3 postdoctoral positions in Bielefeld University (Germany), Aalto University (Finland) and Université catholique de Louvain (Belgium).
In 2015 she got a European Marie Sk{\l}odowska-Curie Fellowship (Project ID: 659104) at the University of Birmingham (UK) before joining the RUG in 2016 as Assistant professor and Rosalind Franklin Fellow. 
She was partner in the European ITN: SUNDIAL (721463), and node leader in DTN EDUCADO (101119830), as well as PI of an NWO VIDI, Smart Industry and HighTech industry projects. 
Bunte's recent work has focused on the development of interpretable and/or efficient machine learning techniques for interdisciplinary data analysis with the principled inclusion of expert knowledge in form of dynamic models with applications in medicine, astronomy and smart industry. %and visualization.  
Further information can be obtained from http://www.cs.rug.nl/$\sim$kbunte/.
\end{IEEEbiography}

% if you will not have a photo at all:
%\begin{IEEEbiographynophoto}{John Doe}
%Biography text here.
%\end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}
